ACTC: Active Threshold Calibration for Cold-Start Knowledge Graph Completion

Self-supervised knowledge-graph completion (KGC) relies on estimating a scoring model over (entity, relation, entity)-tuples, for example, by embedding an initial knowledge graph. Prediction quality can be improved by calibrating the scoring model, typically by adjusting the prediction thresholds using manually annotated examples. In this paper, we attempt for the first time cold-start calibration for KGC, where no annotated examples exist initially for calibration, and only a limited number of tuples can be selected for annotation. Our new method ACTC finds good per-relation thresholds efficiently based on a limited set of annotated tuples. Additionally to a few annotated tuples, ACTC also leverages unlabeled tuples by estimating their correctness with Logistic Regression or Gaussian Process classifiers. We also experiment with different methods for selecting candidate tuples for annotation: density-based and random selection. Experiments with five scoring models and an oracle annotator show an improvement of 7% points when using ACTC in the challenging setting with an annotation budget of only 10 tuples, and an average improvement of 4% points over different budgets.

==> chapters/02_questions.tex <==
\section{Questions}

TODO

We pose several questions which could help us to understand what influences the quality of triple classification systems.

\begin{itemize}
    \item Global/per-relation thresholds?
    \item Towards what metric should we optimize?
    \item Should additional samples be annotated? (with e.g. a simple model trained)
    \item Which samples should be selected for manual annotation? Does the model profit from a more sophisticated samples selection (i.e. not random one)?
\end{itemize}

==> chapters/05_logreg_optimizer.tex <==
\section{Prediction-Based Optimizers}

In this section, we present our new method \name that refines the threshold which is later used for deciding whether to include new triples in the knowledge base (\textit{decision threshold}).
The proposed method can be viewed as an active learning method but has some significant differences.

Firstly, the samples for manual annotation are selected so that the system can benefit the most from their annotation. 
Instead of random selection, \name provides the several selection mechanisms based on the distances between samples and/or their uncertainty estimation (according to the model trained on the manually labeled in the previous iterations data samples). 

Secondly, \name can additionally estimate the labels for new samples and use them with the manually labeled ones for the threshold prediction.

\paragraph{Which samples should be selected for manual annotation?}

In \name the samples which are provided for the annotation and later used as gold samples can be selected in different ways:
\begin{enumerate}
    \item \textbf{randomly}: the samples are selected randomly as in the naive active learning setting;
    \item \textbf{by uncertainty}: first, the model (WHICH ONE) predicts the scores for all the samples, and second, \emph{n} samples the model was the most uncertain about (i.e., their scores are the closest to 0.5) are selected;
    \item \textbf{by density}: the samples which are the closest to the other samples are selected;
    \item \textbf{by density-weighted uncertainty}: a combination of methods (2) and (3), where the sample densities from method (3) are used as weights for the model predicted scores from method (2). 
\end{enumerate}




==> chapters/09_drafts.tex <==
% We adopted it for our setting in the following way. 
%Instead of iteratively trying out the scores of all relevant (i.e., that include the specific relation) triples from the validation set, our Accuracy Optimizer checks only the scores of relevant validation samples from the ones selected on the current algorithm iteration as \textit{gold} samples. 
%For the relations that do not have corresponding samples in the gold samples set, the default threshold is selected from all the samples processed so far as gold ones.
% The original method \cite{safavi-koutra-2020-codex} estimates the relation-specific thresholds: for each relation, a specific threshold is derived from the scores of only the validation triples which contain this relation. 
% In our Accuracy Optimizer, the relation-specific thresholds are selected similarly. Still, the triples with each relation, again, are selected not from the whole validation set but from the current \textit{gold} ones only. 
%Additionally, we provide a \textbf{Global Accuracy Optimizer}, where one global threshold is selected for the whole dataset from the scores of all samples selected as the gold ones on the current algorithm step. 
%The pseudocode for both Accuracy and Global Accuracy Optimizers is provided in Appendix XXX. 



%The proposed method can be viewed as an active learning method but has some significant differences.

%In \name the samples which are provided for the annotation and later used as gold samples can be selected in different ways:
%\begin{enumerate}
    %\item \textbf{randomly}: the samples are selected randomly as in the naive active learning setting;
    %\item \textbf{by uncertainty}: first, the model (WHICH ONE) predicts the scores for all the samples, and second, \emph{n} samples the model was the most uncertain about (i.e., their scores are the closest to 0.5) are selected;
    %\item \textbf{by density}: the samples which are the closest to the other samples are selected;
    %\item \textbf{by density-weighted uncertainty}: a combination of methods (2) and (3), where the sample densities from method (3) are used as weights for the model predicted scores from method (2). 
%\end{enumerate}



==> chapters/draft_02_related_works.tex <==

\section{Related Works}

The KGC problem is usually formulated as a binary triple classification task \cite{Socher2013} whether the candidate triples are classified as correct (i..e, worth being included in the KG) or false based on the triple scores calculated with a KGE model \cite{DBLP:journals/corr/DettmersMSR17, pmlr-v48-trouillon16, NIPS2013_1cecc7a7}. 
However, the scores directly provide only the \textit{ranking} of the candidate triples \cite{DBLP:journals/corr/abs-2111-11845}.
% in order to turn it into \textit{classification} the decision thresholds have to be estimated.
% estimating the quality of the scores with mean reciprocal rank \cite{DBLP:journals/corr/abs-2111-11845}
The problem, which was payed little to no attention for a long time \cite{speranskaya}, is finding a proper \textit{decision threshold} for transforming the scores into class predictions.
% The decision threshold estimation task remained overlooked for a long time \cite{speranskaya}
This task demands additional effort, e.g. a careful creation of additional negative samples \cite{pezeshkpour2020revisiting, safavi-koutra-2020-codex, speranskaya} and often avoided: e.g., instead of direct threshold estimation, the top $k$ samples are selected from the ranked list \cite{choi}, or selection mechanism is modeled in some specific way \cite{dong-etal-2021-docoie}.
%\citet{dong-etal-2021-docoie} use the geometrical setting and classify the candidate triples using $n$-balls constructing methods instead of direct threshold estimation; 
Our method ACTC follows the approach of \citet{safavi-koutra-2020-codex}, who provide the threshold estimation basing on the scores of manually annotated samples. 
In contrast to their approach, ACTC increases the decision sets by additional leveraging of unlabeled data and includes more careful selection of samples for manual annotation. 
% However, this method can estimate only the samples that contain the already known relations.
% In contrast, our method ACTC allows classifying (and, therefore, potential including to the KG) the candidate triples that contain a new for the KB relation.
Our method bears similarity to the active learning, especially its few-shot setting, where the human input is also minimal and highly valued \cite{10.1007/978-3-031-08473-7_9, Pezeshkpour2020OnTU}. 
TODO SO WHAT

% In this paper, we analyze the KGC task as a cold-start problem we analyse in this paper bears similarity to the active learning setting, where the human input is also minimal and highly valued.  







% no "automatically annotated" -> aut labeel

% samples according to informativeness

==> tables/ablation_diff_selection.tex <==
\begin{table}[h!]
\centering
\small
\begin{tabular}{l|cc|cc}
\hline
\multicolumn{1}{c}{}
& \multicolumn{2}{|c}{CoDEx-s}
& \multicolumn{2}{|c}{CoDEx-m}\\
\hline
& LR & GP & LR & GP \\
\hline
random  & 75.75\% &  & 73.0\% & \\
density & -1.25   &  & -1.5 & \\
uncertainty &&&& \\
density-uncertainty &&&& \\
\hline
\end{tabular}
\caption{
Performance (accuracy in \%) of selection mechanisms, averaged over all experiments and KGE models.
}
\label{tab:ablation_sel_mech}
\end{table}

==> tables/results_conve.tex <==
\begin{table}[h!]
\centering
\small
\begin{tabular}{l|rr|rr|rr}
\multicolumn{1}{l}{} &
\multicolumn{2}{|c}{CoDEx-s} & 
\multicolumn{2}{|c}{CoDEx-m} & 
\multicolumn{2}{|c}{14k-QAQ}\\
\hline
\hline
& Acc & F1 & Acc & F1 & Acc & F1 \\
\hline
$AccOpt$ & 99.9 & 99.9 & 99.9 & 99.9 & 99.9 & 99.9 \\
$F1Opt$ & 99.9 & 99.9 & 99.9 & 99.9 & 99.9 & 99.9 \\
$RSTOpt$ & 99.9 & 99.9 &  99.9 & 99.9 & 99.9 & 99.9 \\
\hline
$\name_{1}$ & 99.9 & 99.9 &  99.9 & 99.9 & 99.9 & 99.9 \\
$\name_{10}$  & 99.9 & 99.9 &  99.9 & 99.9 & 99.9 & 99.9 \\
$\name_{avg}$ & 99.9 & 99.9 &  99.9 & 99.9 & 99.9 & 99.9 \\
\hline
%\hline
%CoDEx-s &  32,888 & 3,654 &  3,656 & 2,034 & 42 \\
%CoDEx-m & 185,584 &  20,620 & 20,622 & 17,050 & 51\\
%14k-QAQ &         &         &        &  & \\
%\hline
\end{tabular}
\caption{
Experimental results averaged across all iterations and reported with standard error of the mean. 
% Datasets statistics.  
% The training sets contain only positive triples.
% The ratio of positive to negative samples in validation and test sets: 1:1 for CoDEx-s and CoDEx-m
%Coverage is computed on the train set by dividing the number of samples having at least one match by the number of samples. 
}
\label{table:dataset_stats}
\end{table}

==> tables/results_depr.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{lllllllllllllllllllllllllllllllllllllllll}
\multicolumn{10}{c}{CodEX-s}
& \multicolumn{10}{c}{CodEX-m}
& \multicolumn{10}{c}{14k-QAQ}
& \multicolumn{10}{c}{Avg} &  \\

\multicolumn{2}{l}{RESCAL} 
& \multicolumn{2}{l}{TransE} 
& \multicolumn{2}{l}{Compex} 
& \multicolumn{2}{l}{ConvE} 
& \multicolumn{2}{l}{TuckER} 
& \multicolumn{2}{l}{RESCAL} 
& \multicolumn{2}{l}{TransE} 
& \multicolumn{2}{l}{Complex} 
& \multicolumn{2}{l}{ConvE} 
& \multicolumn{2}{l}{TuckER} 
& \multicolumn{2}{l}{RESCAL} 
& \multicolumn{2}{l}{TransE} 
& \multicolumn{2}{l}{Complex} 
& \multicolumn{2}{l}{ConvE} 
& \multicolumn{2}{l}{TuckER} 
& \multicolumn{2}{l}{RESCAL} 
& \multicolumn{2}{l}{TransE} 
& \multicolumn{2}{l}{Complex} 
& \multicolumn{2}{l}{ConvE} 
& \multicolumn{2}{l}{TuckER} & \\
Acc          & F1          & Acc          & F1          & Acc          & F1          & Acc          & F1         & Acc          & F1          & Acc          & F1          & Acc          & F1          & Acc           & F1          & Acc          & F1         & Acc          & F1          & Acc          & F1          & Acc          & F1          & Acc           & F1          & Acc          & F1         & Acc          & F1          & Acc          & F1          & Acc          & F1          & Acc           & F1          & Acc          & F1         & Acc          & F1          &  \\
             &             &              &             &              &             &              &            &              &             &              &             &              &             &               &             &              &            &              &             &              &             &              &             &               &             &              &            &              &             &              &             &              &             &               &             &              &            &              &             &  \\
             &             &              &             &              &             &              &            &              &             &              &             &              &             &               &             &              &            &              &             &              &             &              &             &               &             &              &            &              &             &              &             &              &             &               &             &              &            &              &             & 
\end{tabular}
\end{table*}
